Understanding Anomaly Detection with Deep Invertible Networks through Hierarchies of Distributions and Features

Deep generative networks trained via maximum likelihood on a natural image dataset like CIFAR10 often assign high likelihoods to images from datasets with different objects (e.g., SVHN). We refine previous investigations of this failure at anomaly detection for invertible generative networks and provide a clear explanation of it as a combination of model bias and domain prior: Convolutional networks learn similar low-level feature distributions when trained on any natural image dataset and these low-level features dominate the likelihood. Hence, when the discriminative features between inliers and outliers are on a high-level, e.g., object shapes, anomaly detection becomes particularly challenging. To remove the negative impact of model bias and domain prior on detecting high-level differences, we propose two methods, first, using the log likelihood ratios of two identical models, one trained on the in-distribution data (e.g., CIFAR10) and the other one on a more general distribution of images (e.g., 80 Million Tiny Images). We also derive a novel outlier loss for the in-distribution network on samples from the more general distribution to further improve the performance. Secondly, using a multi-scale model like Glow, we show that low-level features are mainly captured at early scales. Therefore, using only the likelihood contribution of the final scale performs remarkably well for detecting high-level feature differences of the out-of-distribution and the in-distribution. This method is especially useful if one does not have access to a suitable general distribution. Overall, our methods achieve strong anomaly detection performance in the unsupervised setting, and only slightly underperform state-of-the-art classifier-based methods in the supervised setting. Code can be found at https://github.com/boschresearch/hierarchical_anomaly_detection.

==> hypothesis.tex <==
\section{Common Low-Level Features Dominate the Model Likelihood}

The following hypotheses synthesized from the findings of prior work motivate our methods to detect if an image is from a different object recognition dataset:
\begin{enumerate}[topsep=0pt,parsep=1pt]
    \item Low-level image features contribute the most to the overall likelihood assigned by a deep generative network to any image.
    \item The learned distributions of these low-level features form a domain prior valid for all natural images and do not distinguish well between image distributions of different object categories. 
    \item How strongly which type of features contributes to the likelihood is influenced by the model bias (e.g., for convolutional networks, local features dominate).
    \item Due to the large low-level feature contribution, the likelihood of such models does not distinguish image distributions of different object categories.
\end{enumerate}
\dan{to the the order would be 1, 3, 2, 4. also from 2 to 4, I would say due to the domain piror instead of low level features.}
%We  present some additional findings these hypotheses can explain. Due to the prior works' focus on Glow networks, we also focus on them in this study. \dan{being mentioned in intro}

\dan{It would be nice to mention the corresponding bullet point you summarized. Or for each experiment, you state which bullet of the hypothesis, you want to validate. For instance, the first case, is to check the existence of domain prior}
Glow networks trained independently on CIFAR10, CIFAR100, SVHN or 80 Million Tiny Images (Tiny) produce highly correlated image likelihoods when evaluated on  a diverse set of test images (all pairs of models have spearman-correlations >0.97 for images of aforementioned datasets and LSUN, CelebA and Tiny Imagenet). The same is true to a lesser degree for Fashion-MNIST and MNIST (spearman-correlation 0.80). This suggests they learn a similar domain prior of natural images from the different datasets.\dan{why here you dont cite fig 1?}

\dan{this one shows domain prior locates at early scales, if here you can link to the likelihood decomposition by saying early scales domainate likelhood, then we also show domain prior domiant lokelihood}
Glow networks trained on local patches correlate with models trained on original images. When training modified Glow networks on 8x8 patches cropped from the original images of the datasets, the correlations with the full Glow networks remain larger than 0.97 in the rgb-datasets and above 0.79 for Fashion-MNIST/MNIST. This suggests the correlations of the normal Glow networks can in large parts be attributed to local features.  

\dan{here missing my favorite fig 3, where you show domain prior is low level features, e.g., smoothness. at least should mention fig 2}

\dan{this shows the model bias}
The correlations change for fully connected networks. When training a modified Glow network [see supp] that uses fully connected instead of convolutional blocks on Fashion-MNIST and MNIST, the image likelihoods among them correlate much less (spearman correlation 0.55). The fully-connected Fashion-MNIST network achieves worse likelihoods (4.8 bpd compared to 2.9 bpd), but is much better at anomaly detection (80\% AUROC for Fashion-MNIST vs. MNIST vs 15\% AUROC for convolutional Glow network). %For the rgb-datasets, the reduction in correlation is much smaller (0.97 vs. 0.99)  and the anomaly detection performance remains below chance in difficult cases (e.g. CIFAR10 vs SVHN). 

Taken together, the evidence suggests generative networks have model biases that guide them to learn low-level feature distributions of natural images (domain prior) well, at the expense of anomaly detection performance.\dan{miss mentioning where low-level features locates.} Next, we propose two alternative methods to remove this influence of model bias and domain prior.



==> method.tex <==
\section{Method}\label{sec:method}
We propose two methods for anomaly detection using Glow networks~\citep{NIPS2018_8224}, a state-of-the-art invertible-network architecture. Our first method uses the log likelihood difference of two Glow networks, one trained on the in-distribution, called $G_{\mathrm{in}}$, and the other on 80 million Tiny Images (called  $G_{\mathrm{g}}$) as a general distribution of natural images. From a view of a hierarchy of distributions, we try to remove the effect of the domain prior that is common to all natural images on the log likelihoods attained by $G_{\mathrm{in}}$, by subtracting the log likelihoods attained by $G_{\mathrm{g}}$. Using a Glow network instead of using PNG as in~\citep{Serra2020Input} alleviates the influence of the model bias on the resulting log-likelihood difference of the two Glow-networks. Additionally, we introduce a novel outlier loss to further improve the log-likelihood difference as an anomaly detection metric. The default setting of our method is unsupervised. Its extension to the supervised setting is introduced at the end of the section. Alternatively, our second method exploits the high-level features extracted by the Glow-models for anomaly detection, as Fig.~\ref{fig:anomaly-overview} has shown that they are more in-distribution dependent than low-level features. 

\subsection{Glow model}
Exploiting the available code implementation of Glow models\footnote{\url{https://github.com/y0ast/Glow-PyTorch}}, we construct a Glow model with three scales, see supp. material for the architecture details. The Glow model maps input $x$ onto a latent code $z$, which has the same dimension as $x$ and follows the standard normal distribution denoted as $p_{\mathrm{z}}(z)$. Different to common deep neural networks, such mapping is bijective, i.e., $z=f_G(x)$ and  $x=f_G^{-1}(z)$.
Through variable interchange in $p_{\mathrm{z}}(z)$, the density of $x$ induced by the Glow-model $G$ can be expressed as
\begin{equation}
    p(x)  = p_{\mathrm{z}}(z=f_G(x))\left| \mathrm{det} \left( \frac{\partial f_G(x)}{\partial x} \right) \right|.\label{px}
\end{equation}
$G$ is then trained to maximize $\log p(x)$ on the given training set. The model trained on the in-distribution and a more general distribution, i.e., 80 Million Tiny Images in our cases, is respectively denoted as $G_{\mathrm{in}}$ and $G_{\mathrm{g}}$.

\subsection{Log-likelihood difference}\label{subsec:loglikelihoodratio}
We use the log-likelihood difference of the two Glow-networks, i.e., $G_{\mathrm{in}}$ and $G_{\mathrm{g}}$,  for anomaly detection. Instead of only using the density $p_{\mathrm{in}}(x)$ learned from the in-distribution training inputs, we use its ratio with respect to the density $p_{\mathrm{g}}(x)$ learned from the general distribution inputs, and conveniently evaluate it in the log-domain:
\begin{equation}
\log\left(\frac{p_{\mathrm{in}}(x)}{p_{\mathrm{g}}(x)}\right)=\log\left(p_{\mathrm{in}}(x)) - \log(p_{\mathrm{g}}(x)\right).
\label{eq:likelihooddiff}
\end{equation}
From a compression perspective, the log-likelihood difference is also the difference of the encoding sizes of $x$ respectively attained by $G_{\mathrm{in}}$ and $G_{\mathrm{g}}$. Since $G_{\mathrm{in}}$ is specifically optimized towards compressing inliers while $G_{\mathrm{g}}$ is not, large bit savings, i.e., large log-likelihood difference, are expected for $x$ being inliers. On the other hand, both $G_{\mathrm{in}}$ and $G_{\mathrm{g}}$ rely on the domain priors, respectively learned from the in-distribution and general distribution to encode outliers. We therefore expect reduced or even negative bit savings for outliers. In short, using the log-likelihood difference, anomaly detection is based on the achievable bit savings. 


\subsection{Outlier loss}
\label{subsec:outlier-loss}
We further derive a novel outlier loss for reducing the bit savings on the outliers. Concretely, the log-likelihood difference after temperature scaling by $T$ is used as the logit for binary classification. By the training goal of $G_{\mathrm{in}}$, inliers tend to yield positive logits. Analogous to~\citep{hendrycks2018deep}, we then use 80 Million Tiny Images, i.e., $\{x_{\mathrm{g}}\}$, also for training $G_{\mathrm{in}}$, as the negative class, so the cross entropy loss for them is given as
\begin{align}
L_{\mathrm{o}}=-\lambda\cdot\log\left(\frac{\sqrt [T]{p_{\mathrm{g}}(x_{\mathrm{g}})}}{\sqrt[T]{p_{\mathrm{in}}(x_{\mathrm{g}})} + \sqrt[T]{p_{\mathrm{g}}(x_{\mathrm{g}})}}\right),
\label{eq:negative-loss}
\end{align}
where $\lambda$ is the weighting factor. In the next section, we will compare our outlier loss with the one proposed by~\citeauthor{hendrycks2018deep}  termed margin-based loss.

\subsection{Finetuning}
After training the general distribution Glow-network $G_{\mathrm{g}}$, the learned domain information forms a good starting point for training the in-distribution Glow-network $G_{\mathrm{in}}$. Therefore, here we explore the training of $G_{\mathrm{in}}$ as finetuning the trained $G_{\mathrm{g}}$ on the in-distribution, and further compare it with training from scratch in the next section.


\subsection{Extension to the supervised setting}
\label{ref:methods-supervised}
In all previous parts, our method is presented in an unsupervised setting, where the labels of the inliers are unavailable. Now, we briefly discuss its extension to the supervised setting. It involves two main changes in our training. First, the Glow model $G_{\mathrm{in}}$ uses a mixture of Gaussians for the latent $z$, i.e., each class corresponding to one mode. Second, the outlier loss is extended for each mode of $G_{\mathrm{in}}$ by treating samples from the other classes as the negative samples, i.e., the same as $\{x_{\mathrm{g}}\}$ in (\ref{eq:negative-loss}).


\subsection{Last-scale log likelihood}
\label{subsec:methods-scales}
Our Glow-network has three scales. At the first two scales, i.e., $i=1$ and $2$, the layer output is split into two parts, i.e., $h_i$ and $z_i$, where $h_i$ is passed onto the next scale and $z_i$ is output as one part of the latent code $z$. The output at the last scale is $z_3$, which together with $z_1$ and $z_2$ makes up the complete latent code $z$. In terms of $y_1=(h_1,z_1)$, $y_2=(h_2,z_2)$, $y_3=z_3$ and $h_0=x$, the logarithm of the density $p(x)$ given in (\ref{px}) can be decomposed as
\begin{equation}
\log p(x) = \sum_i \log p_{\mathrm{z}}(z_i) + \log \left| \mathrm{det} \left(\frac{\partial y_i}{\partial h_{i-1}} \right) \right|\label{loglikelihoodscale}.
\end{equation}
In above, the decomposition of $\log p_{\mathrm{z}}(z)$ is because the prior distribution of $z$ assumes mutual independence between $z_1$, $z_2$ and $z_3$, while the chain rule of gradient tells the decomposition of the log-determinant. According to (\ref{loglikelihoodscale}), we can evaluate the log-likelihood, or equivalent encoding size, on each scale, e.g., as shown in Fig.~\ref{fig:anomaly-overview}.


==> method_v1.tex <==
\section{Method}
\subsection{Hierarchy of Distributions}
\begin{figure*}
    \centering
    \includegraphics[scale=0.45]{figures/AnomalyHierarchyDistributions5autocrop.pdf}
    \caption{Overview of the hierarchy-of-distributions log-likelihood differences approach. \textbf{Left}: Schematic hierarchical view of some image distributions. To approximate the distribution of natural images, we use 80 Million Tiny images (Tiny). \textbf{Right}: Results of Glow networks trained on CIFAR10, SVHN and Tiny. Leftmost scatter plots show that the encoding sizes perfectly rank-correlate for all three datasets for the Glow networks trained on CIFAR10 and Tiny, while rank correlation remain very close to 1  between CIFAR10-Glow and SVHN-Glow, validating that the main contribution to the encoding sizes comes from the domain prior. Middle distribution plots show almost identical plots for CIFAR10 and Tiny-Glow and a very low area under the receiver operating curve (AUC) for CIFAR10 vs. SVHN anomaly detection. In contrast, using the encoding size difference between CIFAR10-Glow and Tiny-Glow  reaches substantially higher AUCs, which can be further increased by adding our proposed outlier loss (see Section \ref{subsec:outlier-loss}).
    }
    \label{fig:anomaly-overview_a}
\end{figure*}

Analyzing the models likelihoods more in detail, we find that the models trained on Tiny have the highest average likelihood across all evaluated datasets. This inspired us to use a a hierarchy of distributions: CIFAR10 and SVHN are subdistributions of natural images, CIFAR10-planes are a subdistribution of CIFAR10, etc. (see Fig. \ref{fig:anomaly-overview_a}).

We use this hierarchy of distributions to derive a likelihood-ratio-based anomaly detection method:

\begin{enumerate}[noitemsep,topsep=0pt,parsep=0pt]
    \item Train a generative network on a general image distribution like 80 Million Tiny Images
    \item Train another generative network on images drawn from the in-distribution, e.g., CIFAR10
    \item Use their likelihood ratio for anomaly detection
\end{enumerate}

Given density $p_g$ from the network trained on the general distribution and density  $p_g$ from the network trained on the specific in-distribution, we use their log-likelihood difference as the anomaly metric:
\begin{equation}
\log\left(\frac{p_{\mathrm{in}}(x)}{p_{\mathrm{g}}(x)}\right)=\log\left(p_{\mathrm{in}}(x)) - \log(p_{\mathrm{g}}(x)\right).
\label{eq:likelihooddiff}
\end{equation}

\subsection{Related Methods}
Our method relates to likelihood-ratio based prior \citep{ren_likelihood_ratio} and concurrent \citep{Serra2020Input} methods as follows. \citet{ren_likelihood_ratio} use a noised version of the in-distribution as the general distribution. Their method requires training of two models for each in-distribution, we only require one training of a general distribution model which we can reuse for any new in-distribution. We show improved results over their already strong results in . In our method, the challenge is to find a suitable general distribution, while in their method the challenge is to find a suitable noise model. \citet{Serra2020Input} use a generic lossless compressor such as PNG as their general distribution model and unfortunately only reported results on the training set of the in-distribution, making their results incomparable with any other works. We show improved performance over a reimplementation in supp..

\subsection{Outlier Loss}
We also derive a novel outlier loss on samples from the more general distribution based on the two networks likelihoods.  Concretely, the log-likelihood difference after temperature scaling by $T$ is used as the logit for binary classification:
\begin{equation}
L_{\mathrm{o}}=-\lambda\cdot\log\left(\sigma\left(\frac{log(p_{g}(x_g)) - log(p_{in}(x_g))}{T}\right)\right)=-\lambda\cdot\log\left(\frac{\sqrt [T]{p_{\mathrm{g}}(x_{\mathrm{g}})}}{\sqrt[T]{p_{\mathrm{in}}(x_{\mathrm{g}})} + \sqrt[T]{p_{\mathrm{g}}(x_{\mathrm{g}})}}\right),
\label{eq:negative-loss}
\end{equation}
where $\sigma$ is the sigmoid function and $\lambda$ is a weighting factor. See supplementary for pseudocode.

\subsubsection{Related Methods}
\citep{hendrycks17baseline} used a different margin loss on images from a known outlier distribution (Tiny without CIFAR-images). Therefore, our method can be viewed as a combination of their idea of an outlier loss with our idea of a hierarchy of distributions, and we show improved performance in the unsupervised setting in  ...

\subsubsection{Extension to the Supervised Setting}
In all previous parts, our method is presented in an unsupervised setting, where the labels of the inliers are unavailable. Now, we briefly discuss its extension to the supervised setting. It involves two main changes in our training. First, the Glow model $G_{\mathrm{in}}$ uses a mixture of Gaussians for the latent $z$, i.e., each class corresponding to one mode. Second, the outlier loss is extended for each mode of $G_{\mathrm{in}}$ by treating samples from the other classes as the negative samples, i.e., the same as $\{x_{\mathrm{g}}\}$ in (\ref{eq:negative-loss}).

\subsection{Hierarchy of Features}
\dan{shall we additionally pitch it as if general distribution is not there, this would be alternative. The existence of general distributions has been a common concern of the work in icml.}
\begin{figure*}
    \centering
    \includegraphics[scale=0.5]{figures/AnomalyDetectionHierarchyFeatures3autocrop.pdf}
    \caption{Overview of the hierarchy of features motivation. \textbf{Left}: Showcasing features at different scales in the Glow-network. Top two images are examples from CIFAR10 and SVHN . Bottom two images are obtained by mixing features in the Glow-network trained on CIFAR10 as follows. We compute the three scale outputs of the Glow-network $z_1$, $z_2$ and $z_3$, mix them between both images and invert again. For the bottom-left image, we take the earlier-scale features $z_1$ and $z_2$ from the SVHN image and the final-scale features $z_3$  from the CIFAR10 image and vice versa for the bottom-right image. Note that the image class is completely determined by  $z_3$ . \textbf{Right}: We use two Glow models trained on CIFAR10 and SVHN, respectively.  The log likelihood they obtain on CIFAR10 and SVHN is split into log likelihood contributions of $z_1$, $z_2$ and $z_3$. The two plots show that (i) the summed contributions for $z_1$ and $z_2$ have very high rank correlation between both models; while the rank correlation drops for $z_3$ and (ii) the range of the contributions is much larger for $z_1$ and $z_2$, showing that $z_1$ and $z_2$ dominate the total log likelihood.}
    \label{fig:anomaly-overview}
\end{figure*}

The image likelihood correlations between models trained on different datasets reduce substantially when evaluating the likelihood contributions of the final scale of the Glow network. Note that the glow network has three scales.  At the first two scales, i.e., $i=1$ and $2$, the layer output is split into two parts, i.e., $h_i$ and $z_i$, where $h_i$ is passed onto the next scale and $z_i$ is output as one part of the latent code $z$.  The output at the last scale is $z_3$, which together with $z_1$ and $z_2$ makes up the complete latent code $z$. In terms of $y_1=(h_1,z_1)$, $y_2=(h_2,z_2)$, $y_3=z_3$ and $h_0=x$, the logarithm of the learned density $p(x)$  can be decomposed as
\begin{equation}
\log p(x) = \sum_i \log p_{\mathrm{z}}(z_i) + \log \left| \mathrm{det} \left(\frac{\partial y_i}{\partial h_{i-1}} \right) \right|\label{loglikelihoodscale}.
\end{equation}
According to (\ref{loglikelihoodscale}), we can evaluate the log-likelihood contribution of each scale. The log-likelihood contribution of the final scales of Glow networks correlate substantially less than the full likelihoods for Glow networks trained on the different datasets (0.7 mean correlation vs 0.99 mean correlation).

\subsection{Related Work}
\citet{krusinga2019understanding} developed a method to  approximate probability densities from generative adversarial networks. The densities are computed from a change-of-volume determinant and a latent prior probability density. The latent densities better reflected semantic similarity to the in-distribution than the full density including the determinant.


==> qualitative.tex <==

\subsection{Qualitative Analysis}
Our different metrics (raw likelihoods, log-likelihood ratios and last-scale likelihood contributions) result in qualitatively different highest-scoring images on 80 Million Tiny Images (see Fig. \ref{fig:high-score-tiny} and \ref{fig:high-score-tiny-outlier-loss}). We take a random 120000-images subset of 80 Million Tiny Images and use our Glow network trained on CIFAR10 either with or without outlier loss to compute the  metrics. Looking at the top 12 images per metric shows that using the log-likelihood ratio results in more reasonable images (closer to the inliers) than the raw likelihood, albeit mostly still simple images (see Fig.~\ref{fig:high-score-tiny}) and that using the Glow network trained with outlier loss results in more fitting images for all metrics (see Fig.~\ref{fig:high-score-tiny-outlier-loss}).

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/high_bpd_tiny.png}
    \caption{Most likely images from 80 Million Tiny Images for CIFAR10-Glow.
    12 highest-scoring images selected according to different metrics. First row: raw likelihood, second row: log-likelihood ratio to Tiny-Glow, third row: raw last-scale $z_3$ likelihood contribution. Note that constant images attain the highest raw likelihood, showing the effect of the natural-images domain prior on the raw likelihoods. The highest-scoring log-likelihood-ratio images show a bias towards blue images and some contain actual CIFAR10 objects, namely  birds and planes. Overall, the difference selects some correct images, but is still sensitive to surface features such as the global color. The last-scale results are harder to interpret, the more diverse images suggest it is slightly less affected by the domain prior of smoothness.}
    \label{fig:high-score-tiny}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/high_bpd_tiny_outlier_loss.png}
    \caption{Most likely images from 80 Million Tiny Images for CIFAR10-Glow with the outlier loss. Conventions as in Figure \ref{fig:high-score-tiny-outlier-loss}. Now any of the three metrics lead to selecting mostly CIFAR10-like images, with the log-likelihood difference metric selecting more diverse images with less of a bias towards blueish images.}
    \label{fig:high-score-tiny-outlier-loss}
\end{figure*}




==> related_work.tex <==
\section{Related Work}\label{sec:related-work}
In the literature, there are two general types of anomaly detection methods, one based on discriminative models and the other based on generative models.% , such as training classifiers to be uncertain about outliers; , such as autoencoder- and invertible network-based models to enforce low (ideally zero) density on outliers and high density on inliers. % One takes the discriminative path, e.g., using the softmax response of multi-class classifiers as the indicator for anomaly detection. Following the generative path, the other group either implicitly or explicitly learns the distribution behind in-distribution training samples. Ideally, the learned distribution shall have zero density on any OOD samples. In this paper, our proposal is a generative method as well. It adopts generative invertible networks that are trained to maximize the log-likelihoods of in-distribution training samples. The likelihoods of test samples are used for anomaly detection. Comparing with other generative models, the invertible ones permit to exactly and explicitly evaluate the likelihood of a given data sample. We refer readers to Sec.~\ref{sec:related work} for an overview of related work.
%Discriminative-model based anomaly methods, for instance, use the class probabilities returned by a trained classifier and try to enforce that the probabilities have high-entropy for OOD inputs while retaining low-entropy predictions for in-distribution inputs. Generative model-based anomaly detection methods try to learn the in-distribution from the available training samples. For example, autoencoder based generative models aim at a compact latent representation of the in-distribution and an error-free reconstruction, while OOD samples can suffer from high reconstruction errors and/or yielding outliers in the latent space. Maximum-likelihood-trained generative models try to enforce low likelihoods for OOD and high for in-distribution inputs. 


\textbf{Multi-class Predictive Distribution}~\citeauthor{hendrycks17baseline} empirically showed multi-class classifiers tend to have smaller maximum softmax responses on outliers than inliers. %Therefore, one can exploit the statistics derived from softmax distributions for OOD detection. 
Different data augmentation schemes proposed  respectively by~\citeauthor{liang2018enhancing, lee2018training,hendrycks2018deep,hendrycks2019selfsupervised} further enforced this property for anomaly detection. %, namely, the former adding adversarial perturbations to the inliers and the latter resorting to a generative adversarial network for outlier synthesis. %, namely, adding small adversarial perturbations to the classifier inputs during training, and also by temperature scaling the softmax function. 
%In~\citep{lee2018training}, a GAN was concurrently trained with the classifier to synthesize OOD samples that are close to in-distribution ones. The classifier is then trained to output uniform predictive distribution on such synthesized OOD samples. 
%\citeauthor{hendrycks2018deep} proposed to use dataset that is free to have as the OOD samples to fine-tune the pre-trained classifier, i.e, exposing the classifier to outliers. 
%The recent work by  showed that anomaly detection can benefit from self-supervised training techniques, such as rotating the input image in one of four different degrees and training the network to predict the corresponding rotations.


Instead of using softmax response, \citeauthor{Leenips2018} modeled the class-conditional features attained by the hidden layers of the classifier as multivariate Gaussians, and then use the Mahalanobis distance of Gaussians for anomaly detection. Another recent work~\citep{grathwohl2020your} alternatively evaluated the gradient norm of the log-sum-exp of the class logits over the input for anomaly detection.

\textbf{Input Encoding and Decoding} Another line of work resorts to autoencoder based representation learning and generative modelling, e.g.,~\citep{Pidhorskyi2018,Perera2019OCGANON,abati2019latent}. Briefly, an autoencoder consists of a encoder-decoder pair. The encoder maps the input sample into a latent code that resides in a constrained latent space. As a compact representation of the input, the latent code is fed into a decoder to reconstruct the input. Unlike the inliers on which the autoencoders are trained, outliers tend to suffer from poor reconstruction and low latent code likelihoods. Autoencoders based anomaly detection can greatly benefit from techniques that improve representation learning of the encoder and generative modelling of the decoder.

%Among the generative modelling methods, variational autoencoders and invertible networks explicitly model the data distribution underlying the in distribution training samples. At the test time, whenever the inputs have their densities below a threshold, they are detected as out-of-distribution samples.

%\citep{Choi2020Novelty} augement the training of VQ-VAE with image blurring.

%autoencoder based approaches: \citep{Pidhorskyi2018,Perera2019OCGANON,abati2019latent}

\textbf{Input Likelihood}
%Multi-class classifier attempts to learn the a-posteriori distribution $p(y\vert x)$ of the label $y$ given the input $x$. One important premise for $p(y\vert x)$ being defined is that $x$ must have a positive density, i.e., $p(x)>0$. Therefore, at the test time, it is important to check before classification if every received $x$ has a large enough density. 
Generative models try to enforce high likelihoods on inliers and low (ideally zero) likelihoods on outliers. However, their achieved performance for anomaly detection is still unsatisfactory~\citep{Shafaei2018,nalisnick2018do,hendrycks2018deep}. 
Recent work~\citep{Nalisnick2019DetectingOI} related the poor performance to sampling in a high-dimensional space, namely, inliers being mapped to the typical set of the latent code rather than the high likelihood area. As a result, outliers may attain even higher likelihoods than inliers. They proposed to address this issue by batch-wise anomaly detection, whose application is more limited than instance-wise anomaly detection. 

Concurrent work~\citep{Serra2020Input} to this study showed that input encoding sizes for a trained generative model are more strongly influenced by the input complexity than by whether the input belongs to the training distribution. To remove such influence, they proposed, similar to our approach, to subtract the encoding size produced by a lossless image compressor, such as PNG, from the encoding size produced by the in-distribution generative model. Using the encoding size difference  improves the anomaly detection performance over using the raw encoding size of the in-distribution generative model. 

It is important to note that input complexities in the context of Shannon's source coding theorem is model independent, as it assumes the optimal encoder. On the other hand, the input complexities measured by~\citeauthor{Serra2020Input} are dependent of the models that train on different data distributions as well as general purpose image lossless compressors, such as PNG. When the two encoding sizes, equivalent log-likelihoods, of the same input are measured from two different models, their difference will contain the model bias.




==> related_work_2.tex <==
\section{Related Work}
\label{sec:related-work}

Our hierarchy-of-distributions likelihood-ratio method relates to prior \citep{ren_likelihood_ratio} and concurrent \citep{Serra2020Input} likelihood-ratio methods as follows. \citet{ren_likelihood_ratio} use a noised version of the in-distribution as the general distribution. Their method always requires training of two models for each in-distribution, our method has the option of only require one training of a general distribution model which we can reuse for any new in-distribution as long as it is as a subdistribution of the general distribution. In our method, the challenge is to find a suitable general distribution, while in their method the challenge is to find a suitable noise model. We show improved results over their already good performance in the only rgb-image-setting they evaluate in Section \ref{subsec:logdiff-results}. \citet{Serra2020Input} use a generic lossless compressor such as PNG as their general distribution model and unfortunately only reported results on the training set of the in-distribution, making their results incomparable with any other works. We show improved performance over a reimplementation (code in supp. material) in Section \ref{subsec:logdiff-results}. Note that both works do not evaluate the cases where raw likelihoods work well, even though using the likelihood ratio may decrease performance in that case as seen in Section \ref{subsec:logdiff-results}.

Regarding our outlier loss, \citet{hendrycks2018deep} used a margin loss on images from a known outlier distribution (Tiny without CIFAR-images). Therefore, our method can be viewed as a combination of their idea of an outlier loss with our idea of a hierarchy of distributions, and we show improved performance in the unsupervised setting in Section \ref{subsec:outlier-losses}.

Regarding hierarchy of features, we are not aware of any comparable method directly evaluated for anomaly detection. \citet{krusinga2019understanding} developed a method to  approximate probability densities from generative adversarial networks. The log densities are the sum of a change-of-volume determinant and a latent prior probability density. The latent log densities better reflected semantic similarity to the in-distribution than the full log density, however, no comparable anomaly detection results were reported. \citet{nalisnick2018do} also found the same for latent vs. full log densities of Glow networks, but also did not report anomaly detection results and did not look at individual scales of Glow networks.

One recent state-of-the art purely supervised approach that uses a classifier, adversarial training and generative models is Deep Verifier Networks from~\citet{che2019deepverifier}. This approach outperforms the results reported here, showing that an approach using the class labels without an auxiliary outlier dataset can outperform using 80 Million Tiny Images as outliers. There are two potential reasons for the improved performance. First, they use an adversarial approach, that forces the class-conditional generative model to make its encodings independent of the class label, ensuring the high-level class-discriminative features. They report the importance of this part, consistent with our hypotheses. Second, there are still too many images in Tiny that would be valid CIFAR-images, especially valid images for the people classes in CIFAR100. Therefore, finding a more suitable outlier dataset as well as further improved objective functions are a promising future direction, for both the supervised and unsupervised settings.


==> related_work_3.tex <==
\section{Related Work}
\label{sec:related-work}
We present an overview over anomaly detection approaches with a focus on recent work closely related to the ideas of a hierarchy of distributions and a hierarchy of features.

\textbf{Using a Classifier trained on the Inlier Data}  Classifiers trained to discriminate inlier classes have been used for anomaly detection. ~\citet{hendrycks17baseline} empirically showed multi-class classifiers tend to have smaller maximum softmax responses on outliers than inliers. %Therefore, one can exploit the statistics derived from softmax distributions for OOD detection. 
Different data augmentation schemes proposed respectively in~\citep{liang2018enhancing, lee2018training,hendrycks2018deep,hendrycks2019selfsupervised} further enforced this property. Instead of using the softmax response, \citet{Leenips2018} modeled the class-conditional features attained by the hidden layers of the classifier as multivariate Gaussians, and then used the Mahalanobis distance of Gaussians for anomaly detection.  Another recent work~\citep{grathwohl2020your} alternatively evaluated the gradient norm of the log-sum-exp of the class logits over the input for anomaly detection. A variant to using the original class labels is to train a classifier on a self-supervised pretext task such as discriminating different geometric transformations applied to the inlier images \citep{bergman2020classification,golan2018deep,kim2019rapp}. Later work also combined the ideas of self-supervised contrastive training and using a classifier of the original classes \citep{winkens2020contrastive}.%, namely, the former adding adversarial perturbations to the inliers and the latter resorting to a generative adversarial network for outlier synthesis. %, namely, adding small adversarial perturbations to the classifier inputs during training, and also by temperature scaling the softmax function. 
%In~\citep{lee2018training}, a GAN was concurrently trained with the classifier to synthesize OOD samples that are close to in-distribution ones. The classifier is then trained to output uniform predictive distribution on such synthesized OOD samples. 
%\citeauthor{hendrycks2018deep} proposed to use dataset that is free to have as the OOD samples to fine-tune the pre-trained classifier, i.e, exposing the classifier to outliers. 
%The recent work by  showed that anomaly detection can benefit from self-supervised training techniques, such as rotating the input image in one of four different degrees and training the network to predict the corresponding rotations.



\textbf{Using an Inlier-vs-Outlier Classifier}
A different approach is to explicitly train a classifier function to yield positive values on inliers and negative values on outliers. A prominent example are one-class support vector machines that are trained to return positive values only in a small region containing the training data points and negative values elsewhere \citep{scholkopf2000support}. This approach has also been used in the latent space of deep autoencoders \citep{ruff2018deep,ruff2019deep}, and using samples from a general distribution as outliers \citep{ruff2020rethinking}. In our supplementary, we also show results using a inlier-vs-general-dist classifier in \ref{sec:binary-classifier}. Another variant are methods that explicitly contrast inliers with an artificial distribution like the uniform distribution \citep{steinwart2005classification}. 

\textbf{Using Reconstruction Errors} Another line of work uses autoencoder-based representation learning and generative modelling, e.g.,~\citep{Pidhorskyi2018,Perera2019OCGANON,abati2019latent}. Briefly, an autoencoder consists of a encoder-decoder pair. The encoder maps the input sample into a latent code that resides in a constrained latent space. As a compact representation of the input, the latent code is fed into a decoder to reconstruct the input. For anomaly detection, one expects the inliers to have much lower reconstruction errors than the outliers. Autoencoder-based anomaly detection can greatly benefit from techniques that improve representation learning of the encoder and generative modelling of the decoder.

%Among the generative modelling methods, variational autoencoders and invertible networks explicitly model the data distribution underlying the in distribution training samples. At the test time, whenever the inputs have their densities below a threshold, they are detected as out-of-distribution samples.

%\citep{Choi2020Novelty} augement the training of VQ-VAE with image blurring.

%autoencoder based approaches: \citep{Pidhorskyi2018,Perera2019OCGANON,abati2019latent}

\dan{I wonder if the three papers are better grouped under auto-encoder based representation learning, as they worked due to some smart manipulation on the latent space, \ref{abati2019latent} also latent prior in addition to reconstruction error.}

\textbf{Using Input Likelihoods}
%Multi-class classifier attempts to learn the a-posteriori distribution $p(y\vert x)$ of the label $y$ given the input $x$. One important premise for $p(y\vert x)$ being defined is that $x$ must have a positive density, i.e., $p(x)>0$. Therefore, at the test time, it is important to check before classification if every received $x$ has a large enough density. 
Generative models try to enforce high likelihoods on inliers and are therefore expected to yield low (ideally zero) likelihoods on outliers. However, their anomaly detection performance is often unsatisfactory~\citep{Shafaei2018,nalisnick2018do,hendrycks2018deep}. 
Recent work~\citep{Nalisnick2019DetectingOI} related the poor performance to sampling in a high-dimensional space, namely, inliers being mapped to the typical set of the latent code rather than the high likelihood area. As a result, outliers may attain even higher likelihoods than inliers. They proposed to address this issue by batch-wise anomaly detection, whose application is more limited than instance-wise anomaly detection. %Empirically, energy-based models have achieved better anomaly detection performance \citep{zhai2016deep}. 
A different approach called Deep Verifier Networks \citep{che2019deepverifier} combined input likelihoods with inlier classifiers. They trained a class-conditional generative model with an auxiliary adversarial loss to \dan{disentangle the class information from the rest latent representation. The achieved performance is better than our methods in the supervised setting, whereas ours mainly target and work in the unsupervised setting. It can be an interesting future work to improve our methods in the supervised setting by exploiting the way of incorporating the label information as proposed in \citep{che2019deepverifier}.}

Our work also uses input likelihoods, exploiting hierarchies of distributions or hierarchies of features as explained in Section \ref{sec:hierarchy-distributions} and \ref{sec:hierarchy-features} to improve the anomaly detection performance.

%ensure that the learned latent code distributions are indistinguishable between the different classes. Their excellent anomaly detection performance in some cases outperforms the results here, even though no outliers are used during training. The improvements may be because the adversarial component enforces that the generative model uses as much class information as possible or because there are still too many "outlier" images in Tiny that would be valid CIFAR-images. Therefore, finding a more suitable outlier dataset as well as further improved objective functions are a promising future direction, for both the supervised and unsupervised settings. Our work also uses input likelihoods and improves anomaly detection performance by exploiting hierarchies of distributions or hierarchies of features as explained in Sections \ref{sec:hierarchy-distributions} and \ref{sec:hierarchy-features}.

%Concurrent work~\citep{Serra2020Input} to this study showed that input encoding sizes for a trained generative model are more strongly influenced by the input complexity than by whether the input belongs to the training distribution. To remove such influence, they proposed, similar to our approach, to subtract the encoding size produced by a lossless image compressor, such as PNG, from the encoding size produced by the in-distribution generative model. Using the encoding size difference  improves the anomaly detection performance over using the raw encoding size of the in-distribution generative model. 

%It is important to note that input complexities in the context of Shannon's source coding theorem is model independent, as it assumes the optimal encoder. On the other hand, the input complexities measured by~\citeauthor{Serra2020Input} are dependent of the models that train on different data distributions as well as general purpose image lossless compressors, such as PNG. When the two encoding sizes, equivalent log-likelihoods, of the same input are measured from two different models, their difference will contain the model bias.

\textbf{Hierarchy of Distributions} Our hierarchy-of-distributions likelihood-ratio method relates to prior \citep{ren_likelihood_ratio} and concurrent \citep{Serra2020Input} likelihood-ratio methods as follows. \citet{ren_likelihood_ratio} use a noised version of the in-distribution as the general distribution. Their method always requires training of two models for each in-distribution, our method has the option of only require one training of a general distribution model which we can reuse for any new in-distribution as long as it is as a subdistribution of the general distribution. In our method, the challenge is to find a suitable general distribution, while in their method the challenge is to find a suitable noise model. We show improved results over their already good performance in the only rgb-image-setting they evaluate in Section \ref{subsec:logdiff-results}. \citet{Serra2020Input} use a generic lossless compressor such as PNG as their general distribution model and unfortunately only reported results on the training set of the in-distribution, making their results incomparable with any other works. We show improved performance over a reimplementation (code in supp. material) in Section \ref{subsec:logdiff-results}. Note that both works do not evaluate the cases where raw likelihoods work well, even though using the likelihood ratio may decrease performance in that case as seen in Section \ref{subsec:logdiff-results}.

\textbf{Outlier Loss} \citet{hendrycks2018deep} used a margin loss on images from a known outlier distribution (Tiny without CIFAR-images). We develop an outlier loss to improve the performance of likelihood models. It can be viewed as a combination of their idea of an outlier loss with our view of a hierarchy of distributions, and achieved an improved performance in the unsupervised setting in Section \ref{subsec:outlier-losses}.

\textbf{Hierarchy of Features} Regarding hierarchy of features, the closest related work found that in a deep variational autoencoder with a hierarchy of stochastic variables, later stochastic variables perform better at anomaly detection \citep{maaloe2019biva}.\dan{gammer? I could not understand the sentence before.} Furthermore, \citet{krusinga2019understanding} developed a method to  approximate probability densities from generative adversarial networks. The log densities are the sum of a change-of-volume determinant and a latent prior probability density. The latent log densities better reflected semantic similarity to the in-distribution than the full log density, however, no comparable anomaly detection results were reported. \citet{nalisnick2018do} also found the same for latent vs. full log densities of Glow networks, but also did not report anomaly detection results and did not look at individual scales of Glow networks. In contrast to our results, \citet{huang2019out} found that for a CNN trained as part of a generative model, the likelihood of latent variables from all layers performs well for anomaly detection.\dan{if they use all latent variables, why this relates to last scale feature?} In concurrent work, \citet{kirichenko2020why} investigated the anomaly detection behavior of generative convolutional invertible networks and find results consistent with ours, namely that generic local pixel correlations dominate the likelihood.\dan{but they did not suggested look at the last scale. to me, it is related work in the sense of building up the view.}

%One recent state-of-the art purely supervised approach that uses a classifier, adversarial training and generative models is Deep Verifier Networks from~\citet{che2019deepverifier}. This approach outperforms the results reported here, showing that an approach using the class labels without an auxiliary outlier dataset can outperform using 80 Million Tiny Images as outliers. There are two potential reasons for the improved performance. First, they use an adversarial approach, that forces the class-conditional generative model to make its encodings independent of the class label, ensuring the high-level class-discriminative features. They report the importance of this part, consistent with our hypotheses. Second, there are still too many images in Tiny that would be valid CIFAR-images, especially valid images for the people classes in CIFAR100. Therefore, finding a more suitable outlier dataset as well as further improved objective functions are a promising future direction, for both the supervised and unsupervised settings.

